Concentration-Bound Analysis for Probabilistic Programs and Probabilistic Recurrence Relations

Analyzing probabilistic programs and randomized algorithms are classical problems in computer science. The first basic problem in the analysis of stochastic processes is to consider the expectation or mean, and another basic problem is to consider concentration bounds, i.e. showing that large deviations from the mean have small probability. Similarly, in the context of probabilistic programs and randomized algorithms, the analysis of expected termination time/running time and their concentration bounds are fundamental problems.In this work, we focus on concentration bounds for probabilistic programs and probabilistic recurrences of randomized algorithms. For probabilistic programs, the basic technique to achieve concentration bounds is to consider martingales and apply the classical Azuma's inequality. For probabilistic recurrences of randomized algorithms, Karp's classical "cookbook" method, which is similar to the master theorem for recurrences, is the standard approach to obtain concentration bounds. In this work, we propose a novel approach for deriving concentration bounds for probabilistic programs and probabilistic recurrence relations through the synthesis of exponential supermartingales. For probabilistic programs, we present algorithms for synthesis of such supermartingales in several cases. We also show that our approach can derive better concentration bounds than simply applying the classical Azuma's inequality over various probabilistic programs considered in the literature. For probabilistic recurrences, our approach can derive tighter bounds than the Karp's well-established methods on classical algorithms. Moreover, we show that our approach could derive bounds comparable to the optimal bound for quicksort, proposed by McDiarmid and Hayward. We also present a prototype implementation that can automatically infer these bounds

==> popl_main_auto_algo_old.tex <==
\subsection{Automated techniques}

In this part, we illustrate an algorithm that could automatically give upper bound while $\ell = 1$, given probabilistic recurrence relation, tail function$\kappa$ and state function $f$, followed from \yican{cite CAV17Recurrence paper}, we make assumption on the relation, $a(n),\kappa$ and $f(n)$.  We assume that all of $a(n),\kappa$ and $f(n)$ could be described by the following grammar:
\[
	E ::= c\ |\ E + E\  |\  c \times E\ |\ n \ln n\ |\ \ln n\ |\ n
\]
Where $c>0$, we further assume that the PRR follows the grammar below:
\begin{align*}
\mathfrak t ::= &c\ |\ n\ | \ln n\ |\ n\cdot \ln n\ |\  \mathfrak {t} + \mathfrak {t}\ |\  c\times {\mathfrak t} \\
&\ \frac 1n \sum_{i = 0}^{n-1} T(j)\ |\ \frac{1}{n}(\sum_{i = \lfloor n/2\rfloor}^{n - 1} T(i) + \sum_{i = \lceil n/2\rceil}^{n-1} T(i))
\end{align*}

The goal our algorithm would search $\alpha>1$ such that $(Y_m(\alpha))_{m\geq 0}$ is an exponential supermartingale under input $n^*$.

Before the introduction of our algorithm, we first demonstrate some mathematical foundations.
\begin{lemma}
For any monotonically increase function $f$ defined on interval $[l,r+1]$, where $l,r\in \mathbb N$:
$$\sum_{i=l}^r f(x)\leq \int_{l}^{r+1} f(x) \text dx$$
\end{lemma}\label{lemma:summation}

\begin{proof}

By simple calculus. \yican{draft here, I would complete}

\end{proof}

Our algorithm goes as follows:

\textit{1. Derive conditions for $\alpha$}. To apply Lemma \ref{lemm:recurrence}, we should infer conditions for $\alpha$ from program codes. This could be done with the help of \yican{cite CAV17Recurrence paper}.

\begin{example}
Again we set function $f(n):=5n$, so its condition is:
\begin{align*}
\forall n\leq n^*, \alpha^{5\cdot n}&\geq \alpha^{n-1} \cdot \frac{1}{n} \cdot \left(\sum_{i=\lceil n/2 \rceil}^{n-1} \alpha^{5\cdot i} + \sum_{i=\lfloor n/2 \rfloor}^{n-1} \alpha^{5 \cdot i}\right)
\end{align*}
\end{example}


\textit{2. Overapproximate summation}. At first we tackle with the summation term. To begin with, under conditions mentioned above, every summation term would calcuate a sum for a monotonically increase function. By Lemma \ref{lemma:summation}, we would use integration to overapproximate every summation. To tackle with ceils and floors in the result, we would utilize the property of concave function(Note that the antiderivative is always concave) to simplify the result. For functions that has no elementary antiderivative, such as $\alpha^{n\ln n}$, we would partition the summation uniformly into $B$ parts and in each part, we would use the maximum value to overapproximate terms in this part. The number of parts $B$ is automatically determined. In our implementation, we would try $B = 2, 4, 8, \cdots$ one by one until our solver has no ability to solve constraints.

\begin{example}
Continued from the previous example, we would use $\sum_{i=l}^{r}{\alpha^{5i}}\leq \int_{l}^{r+1} \alpha^{5x}\text dx = \frac{\alpha^{5(r+1)} - \alpha^{5l}}{5\ln \alpha}$ to overapproximate two summation terms:
\begin{align*}
\forall n\leq n^*, \alpha^{5\cdot n}&\geq \alpha^{n-1}\cdot  \frac{1}{n}\cdot  \frac{\alpha^{5\cdot n} - \alpha^{5\cdot \lceil n/2\rceil} + \alpha^{5\cdot n} - \alpha^{5\cdot \lfloor n/2\rfloor}}{5\ln \alpha}
\end{align*}

By the concavity of $\alpha^{5\cdot x}$, we could safely simplify the result:
\begin{align*}
\forall n\leq n^*, \alpha^{5\cdot n}&\geq \alpha^{n-1}\cdot  \frac{2}{n}\cdot  \frac{\alpha^{5\cdot n} - \alpha^{2.5\cdot n} }{5\ln \alpha}
\end{align*}

\end{example}

\textit{3. Substitution and simplification}. Here we would introduce a new variable $c:=c(\alpha,n)>1$ to do substitution on this inequality, the form of $c(\alpha,n)$ is determined as $\alpha^{g(n)}$, where $g(n)$ is the highest complexity term in $f(n)$. After substitution, we would firstly remove everything to the leftside of inequality, and to eliminate fractions, we would multiply the denominator(under our assumption, it is always positive). then we consider every terms $a\cdot c^{b\cdot x}$ in the expresssion, if $x$ contains some variable, and if we have $a>0\land b>0$, or $a<0\land b<0$(this is judged by constant), we found that removing this term would not lose soundness but further simplify the inequality, in our implementation, we do this in an eager way, we would eliminate all these terms. 
% we would further simplify the inequality in two aspects: (1) safe multivariate term removals. We would remove all terms that could further strengthen the inequality. (2) safe transpotations to eliminate fractions. We would ensure the denominator of this fraction is always positive(or negative). 

\begin{example}
	
	Now we choose $c:=\alpha^n$, then constraints become (note that $\ln c = n \cdot \ln \alpha$):
	\begin{align*}
	\forall n\leq n^*, c^{5}&\geq c^{1 - 1/n}\cdot \frac{2}n \cdot  \frac{c^5 - c^{2.5}}{5 \ln \alpha}
	\end{align*}
	
	Then we move everything to the left:
	\begin{align*}
	\forall n\leq n^*, c^{5}- c^{1 - 1/n}\cdot \frac{2}n \cdot  \frac{c^5 - c^{2.5}}{5 \ln \alpha}\geq 0
	\end{align*}
	
	Then eliminiate fractions
	
	\begin{align*}
	\forall n\leq n^*, c^{5}\cdot n\cdot 5\cdot \ln \alpha- c^{1 - 1/n}\cdot 2\cdot (c^5 - c^{2.5})\geq 0
	\end{align*}
	
	Note that the term $c^{-1/n}<1$ is on the leftside with negative coeficient, so its removal would strengthen the inequality, so we would remove both terms. 
	\begin{align*}
	\forall n\leq n^*, c^{5}\cdot n\cdot 5\cdot \ln \alpha- c\cdot 2\cdot (c^5 - c^{2.5})\geq 0
	\end{align*}
\end{example}

After 2 steps above, we expect the inequality has the form $\psi(c) \geq 0$, otherwise our algorithm would fail and output $1$ for soundnesss. Now we introduce a lemma to describe the form of $\psi$. \yican{maybe it should be a claim, need to be checked}

\textit{3. Substitution and simplification}. Here we would introduce a new variable $c:=c(\alpha,n)>1$ to do substitution on this inequality, the form of $c(\alpha,n)$ is determined as $\alpha^{g(n)}$, where $g(n)$ is the highest complexity term in $f(n)$. After substitution, we would further simplify the inequality in two aspects: (1) safe multivariate term removals. We would remove all terms that could further strengthen the inequality (2) safe transpotations to eliminate fractions. We would ensure the denominator of this fraction is always positive(or negative).

\begin{example}

Now we choose $c:=\alpha^n$, then constraints become:
\begin{align*}
\forall n\leq n^*, c^{5}&\geq c^{1 - 1/n}\cdot \frac{2}n \cdot  \frac{c^5 - c^{2.5}}{5 \ln \alpha}
\end{align*}

Note that the term $c^{-1/n}<1$ is on the rightside with positive coeficient, so its removal would strengthen the inequality, so we would remove both terms. Moreover, since $n\ln \alpha = 5\ln c > 0$, we could eliminate this fraction by multiplying $5\ln c$ in both sides of inequality. Finally, by moving all rightside terms to the leftside, we derive constraints:
\begin{align*}
\forall n\leq n^*, 5\cdot c^{1.5}\cdot \ln c - 2\cdot c^{2.5} + 2&\geq 0
\end{align*}
\end{example}

After 2 steps above, we expect the inequality has the form $\psi(c) \geq 0$, otherwise our algorithm would fail and output $1$ for soundnesss. Now we introduce a lemma to describe the form of $\psi$. \yican{maybe it should be a claim, need to be checked}
\begin{lemma}
Under the assumptions mentioned above, we claim that $\psi(c)$ should have the following form:
$$\psi(c) = \sum_{i\in \mathcal I} \alpha_i c^{\beta_i} \ln^{n_i} c$$
where $\alpha,\beta_i \in \mathbb R, n_i\in \{0,1\}, \alpha_i\neq 0$. Moreover, this form is closed under derivation, which means if $\psi(c)$ has this form, then $\psi'(c)$ also does.
\end{lemma}\label{lemma:form}

\begin{proof}
Case anaylsis. \yican{draft here, I would complete}
\end{proof}

In this paper, we seek the property \textit{PosNeg($\psi$)} \yican{seek for another name} for function $\psi$: there exists $1\leq c^*\geq \infty$ such that $\psi(c) > 0$ on $(1,c^*)$ and $\psi(c) < 0$ on $(c^*, \infty)$, which would be useful for finding the tail probability in our algorithm, and we establish the following lemma for \textit{PosNeg($\psi$)}:
\begin{lemma}
For smooth function $\psi(c)$, there are two conditions to judge whether \textit{PosNeg($\psi(c)$)} holds.
\begin{itemize}
	\item If $\psi$ is strictly decreasing, and $\psi(1) \geq 0$, then \textit{PosNeg($\psi$)} holds.
	\item If the property \textit{PosNeg($\psi'(c)$)} holds, and $\psi(1) \geq 0$, then \textit{PosNeg($\psi$)} holds.
\end{itemize}
\end{lemma}\label{lemma:PosNeg}

\begin{proof}

\textit{proof of condition 1}. Define $\psi(\infty) := \lim_{t\to \infty} \psi(t)\in \mathbb R \cup \{-\infty\}$.(Note that this value always exsits).
Set $c^*:=\sup\{x|x\geq 1\land \psi(x)\geq 0\}$, then by $\forall x>c^*, \psi(x)<0$. By continuous of $\psi$, we have $\psi(c^*)\geq 0$. since $\psi$ is monotonically decreasing, $\forall x< c^*, \psi(x)> \psi(c^*)\geq 0$, so $c^*$ is feasible.

\textit{proof of condition 2}. Since \textit{PosNeg($\psi'(c)$)} holds, there exists $c'$ such that $\psi'(c)>0$ on $(1,c')$ and $\psi'(c)<0$ on $(c',\infty)$.
By Newton-Lebniz formula: $\psi(c') = \psi(1) + \int_{1}^{c'} \psi'(t) \text{d}t$, we have $\psi(c') \geq \psi(1) \geq 0$. Since $\psi'(c) < 0$ on $(c', \infty)$, then by similar prove with condition $1$, we conclude that \textit{PosNeg($\psi(c)$)} holds.

\end{proof}

\textit{4. Finding non-negative part of univariate function}. Then we prove whether $\psi$ has the property \textit{PosNeg($\psi$)}, if it holds, then we could use binary search to find $c^*$ numerically. We assume $\psi(1) \geq 0$(otherwise this property obviously does not hold), to prove this, we would use Algorithm \ref{alg:property}:
\begin{algorithm}[h]
\small
\LinesNumbered
\caption{Algorithm for proving \textit{PosNeg($\psi$)}}
\KwIn{A function $\psi$ with form in Lemma \ref{lemma:form}}
\KwOut{Whehter $\psi$ satisifes \textit{PosNeg($\psi$)}}
\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{Simp}{Simplify}
\SetKwFunction{MDec}{MonoDec}
\SetKwFunction{Prove}{ProveProperty}
\Fn{\Simp{$\psi = \sum_{i\in \mathcal I} \alpha_i c^{\beta_i} \ln^{n_i} c$}}{
	\uIf{for each $i\in \mathcal I$, $\beta_i\neq 0$}{
		Pick $i_0\in \mathcal I$\\
		\Return $c^{-\beta_{i_0}}f(c)$
	}
	\Return $\psi$
}

\Fn{\MDec{$\psi = \sum_{i\in \mathcal I} \alpha_i c^{\beta_i} \ln^{n_i} c$}}{
	$\psi\leftarrow $ \Simp{$\psi$} \\
	$\psi' := \frac{\text d \psi}{\text d c} = \sum_{i\in \mathcal I'} \alpha'_i c^{\beta'_i} \ln^{n_i'} c$ \\
	\uIf{for each $i\in \mathcal I$, $\alpha_i< 0$}{
		\Return True
	}
	\uIf{$\psi\neq 0\land $\MDec{$\psi'$}$\land \psi'(1) < 0$}{
		\Return True
	}
	\Return False
}
\Fn{\Prove{$\psi = \sum_{i\in \mathcal I} \alpha_i c^{\beta_i} \ln^{n_i} c$}}{
	$\psi\leftarrow $ \Simp{$\psi$} \\
	$\psi' := \frac{\text d \psi}{\text d c} = \sum_{i\in \mathcal I'} \alpha'_i c^{\beta'_i} \ln^{n_i'} c$ \\
	\uIf{\MDec{$\psi$}}{
		\Return True
	}
	\uIf{$\psi\neq 0\land $ \Prove{$\psi'$} $\land \psi'(1) \geq 0$}{
		\Return True
	}
	\Return False
}
\end{algorithm}\label{alg:property}

Function \texttt{simplify} function would do some modification on $\psi$, if every term in this summation has subterm $c^{\beta_i}, \beta_i\neq 0$, then we could simplify this function by dividing one $c^{-\beta_{i_0}}$ to eliminate one of these subterms. Note that this operation preserve the property \textit{PosNeg($\psi$)} and monotonicity.

Function \texttt{MonoDec} function would check whether $\psi$ is strictly decreasing. It would first to simplification on $\psi$, and then do basic checks for $\psi'$.

Function \texttt{Prove} function would check whether $\psi$ satisfies the property \textit{PosNeg($\psi$)} by Lemma \ref{lemma:PosNeg}.

\begin{example}
Continued on previous examples, we have:
\begin{align*}
\psi(c) &= 5c^{1.5}\ln c - 2c^{2.5} + 2\\
\psi'(c) &= 7.5c^{0.5}\ln c+5c^{0.5}-5c^{1.5}\\
\frac{\text d}{\text d c} (\psi'(c) / c ^{0.5}) &= 7.5/c - 5\\
\end{align*}

The procedure is shown below:
\begin{enumerate}
	\item We would firstly found that $\psi(c)$ is not monotone, and then turn to prove \textit{PosNeg($\psi'$)}.
	\item Next we found that $\psi'$ could be simplified by dividing $c^{0.5}$ and becomes $7.5\ln c + 5 - 5c$, we found it is also not monotone, so agiain we turn to prove \textit{PosNeg($\frac{\text d}{\text d c} (\psi'(c) / c ^{0.5})$)} = \textit{PosNeg($7.5/c-5$)}.
	\item We found that $7.5/c-5$ is monotone decreasing, so \textit{PosNeg($7.5/c-5$)} holds.
	\item By evaluating $\psi'(1) = 0$, by Lemma \ref{lemma:PosNeg} we conclude that \textit{PosNeg($f'(c)$)} holds.
	\item By evaluating $\psi(1) = 0$, we conclude that \textit{PosNeg($\psi(c)$)} holds.
\end{enumerate}

\end{example}

\textit{5. Apply Back}. Since we derive that $c\in [1,c^*]\rightarrow \psi(c) \geq 0$, and since for every $\alpha$, $c(\alpha,n)$ increases as $n$ increases. It suffices to find $\alpha$ such that: $c(\alpha,1)\geq 1\land c(\alpha,n^*)\leq c^*$, we would use off-the-shelve solver to solve this function.
\begin{example}

Continued on previous examples, we solved $\psi(c) = 0$ and derive $c^* \approx 2.74$, then it constraints become $\alpha \geq 1 \land \alpha^{n^*}\leq 2.74$, so we would apply $\alpha = 2.74^{\frac{1}{n^*}}$ back to derive the bound:
\end{example}


We establish a theorem for Algorithm \ref{alg:property}:
\begin{theorem}
Under conditions in Section 5.1, Algorithm \ref{alg:property} runs in polynomial time.
\end{theorem}\label{thm:alg} \yican{maybe it should be a claim, need to be checked}

\begin{proof}

By Lemma \ref{lemma:form}, we obatin that every argument of $\psi$ has the form mentioned in Lemma \ref{lemma:form}.
Define $\psi_t(c)$ to be the argument of \texttt{Prove} after $t$-th recursive calls. Assume:
$$\psi_t(c) = \sum_{i} {\alpha_i^{(t)}c^{\beta_i^{(t)}}\ln^{n_i^{(t)}}c}$$

Define $S_t = |\{i|\alpha_i\neq 0\}|$, $L_t = |\{i|n_i\neq 0\}|$, we first prove the depth of recursion would be no larger than $S_1+L_1$.

Then after calling \texttt{simplify} subroutine, then some $i_0$ we have $\beta_{i_0}^{(t)} = 0$, if $n_{i_0}^{(t)} = 0$, then after derivation, this term would vanish, so we have $S_{t+1}\leq S_t - 1$. Otherwise if $n_{i_0}^{(t)} = 1$, then after derivation, this term would be $\alpha_i^{(t)}c^{-1}$, which means $L_{t+1}\leq L_t-1$. Hence, the depth of recursion would be no larger than $S_1+L_1$, which is polynomial to the length of initial input.

Similarly, we could prove that the depth of recursions in \texttt{MDec} has polynomial time complexity. Moreover, every operation in the body of \texttt{Prove} and \texttt{MDec}(such as diffrentiate a function) has polynomial time complexity. Hence we have \ref{alg:property} has polynomial time complexity.


\end{proof}

For our automated technique, we have the following theorem:
\begin{theorem}
Under conditions in Section 5.1, our automated ensures soundness.
\end{theorem}\label{thm:alg} \yican{maybe it should be a claim, need to be checked}

\begin{proof}

Firstly, Algorithm \ref{alg:property} is sound since it strictly follows Lemma \ref{lemma:PosNeg}.

\end{proof}

